Auctions with LLM Summaries

We study an auction setting in which bidders bid for placement of their content within a summary generated by a large language model (LLM), e.g., an ad auction in which the display is a summary paragraph of multiple ads. This generalizes the classic ad settings such as position auctions to an LLM generated setting, which allows us to handle general display formats. We propose a novel factorized framework in which an auction module and an LLM module work together via a prediction model to provide welfare maximizing summary outputs in an incentive compatible manner. We provide a theoretical analysis of this framework and synthetic experiments to demonstrate the feasibility and validity of the system together with welfare comparisons.

==> fine-tuning.tex <==
\section{Fine Tuning LLM}\label{sec:ft-llm}
Why do we need finetuning? For this let us review the assumptions involved in optimizing the objective using prompt engineering. Given a set of creatives $X=\{x_i\}_{i=1}^k$ corresponding to k competing ads, and an associated summary $S$ produced by an LLM, we seek to optimize the expected click through rate:
\begin{equation*}
    CTR(S,X):=\sum_{i=1}^k CTR(S, x_i) \cdot Q(x_i),
\end{equation*}
where, $Q(x_i)$ is the inherent quality of the creative associated with ad $i$, and $CTR(S,x_i)$ is the expected click through rate for ad $i$ based on properties of the summary $S$. In the case of prompt engineering, we assume the $CTR(\cdot)$ of the $i^{th}$ ad is unaffected by the summary associated with other ads beyond a generalized position associated with ad $i$, and which is dictated by position of all other ads (i.e. $CTR(S,x_i)=CTR(S_i,x_i)\cdot CTR(pos_i)$). Furthermore, note that we assume the LLM is capable of following the instructions specified in the prompt, and this goes into the design of the prompt, where, we prompt the LLM "$k$" times and append these outputs to produce the summary in question.

Clearly, for ads with complex formats and dependencies, the CTR of any ad is affected by the properties/content of the entire summary. To model this realistic scenario, we require providing a complex prompt containing all creatives and associated instructions we seek the summary to satisfy. Apriori, one cannot hope to guarantee the LLM to satisfy the constraints encoded in such a prompt. It is in this scenario that we require building empirical models of $CTR(S,x_i)$ and using this to optimize the parameters of the LLM to satisfy the following objectives -\\
(1) maximize total clicks\\
(2a) monotonicity: the order the pctr is similar to the order of prominence, or,\\
(2b) matching relative prominence, i.e. with $\hat{p}_i \propto CTR(S,x_i)Q(x_i)$, minimize $KL(p||\hat{p})$.


==> monotone-llm.tex <==
\section{Monotone LLM}

